Eliminating Network Protocol Vulnerabilities Through Abstraction and Systems Language Design

Incorrect implementations of network protocol message specifications affect the stability, security, and cost of network system development. Most implementation defects fall into one of three categories of well defined message constraints. However, the general process of constructing network protocol stacks and systems does not capture these categorical con- straints. We introduce a systems programming language with new abstractions that capture these constraints. Safe and efficient implementations of standard message handling operations are synthesized by our compiler, and whole-program analysis is used to ensure constraints are never violated. We present language examples using the OpenFlow protocol.

==> IEEEtran/README <==

December 27, 2012


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

V1.8 is a significant update over the 1.7a release. For a full list of
changes, please read the file changelog.txt. The most notable changes
include:


 1) New transmag class option to support the IEEE Transactions on Magnetics
    format. Thanks to Wei Yingkang, Sangmin Suh and Benjamin Gaussens
    for suggestions and beta testing.

 2) The \IEEEcompsoctitleabstractindextext and 
    \IEEEdisplaynotcompsoctitleabstractindextext
    commands have been deprecated in favor of their
    \IEEEtitleabstractindextext and \IEEEdisplaynontitleabstractindextext
    (observe that the "not" has changed to "non") equivalents. This change
    generalizes and decouples them from compsoc mode because the new
    transmag mode also uses them now.

 3) Added new *-forms of \IEEEyesnumber*, \IEEEnonumber*, \IEEEyessubnumber*,
    and \IEEEnosubnumber* (the non-star form of the latter is also new) which
    persist across IEEEeqnarray lines until countermanded. To provide for
    continued subequations across instances of IEEEeqnarrays as well as for
    subequations that follow a main equation (e.g., 14, 14a, 14b ...)
    \IEEEyessubnumber no longer automatically increments the equation number
    on it's first invocation of a subequation group. Invoke both
    \IEEEyesnumber\IEEEyessubnumber together to start a new
    equation/subequation group.
 
 4) Hyperref links now work with IEEEeqnarray equations.
    Thanks to Stefan M. Moser for reporting this problem.

 5) Revised spacing at top of top figures and tables to better
    align with the top main text lines as IEEE does in its journals. 
    Thanks to Dirk Beyer for reporting this issue and beta testing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> background.tex <==
\section{Background}

This work focuses on both stream and datagram oriented protocols with binary
message representations that have value directed interpretations. In this
section we will describe three simple protocol message formats that are
representative of the internal structure and variability of message
representations. We currently do not handle formats that require extensive
pattern matching to determine field types, such as SMTP, HTTP, or SIP. Binary
message formats typically have a self-describing structure; some initial format
is assumed for the prefix of the message, while values within the prefix
determine the format of the rest of the message.

\subsection{OpenFlow Protocol}

We have selected a small subset of message representations found in the OpenFlow
v1.0 protocol specification~\cite{ofp_1_0}. This protocol follows the traditional structure
of a Type-Length-Value (TLV) based representation. There is a fixed size header
for any OpenFlow message that does not vary in structure across all existing
versions of the protocol. The header is comprised of a version, type, length,
and transaction identifier. Most Significant Byte First (MSBF) is the followed
for all multi-byte fields. A message is comprised of the header followed by a
variable payload. The type of the payload is indicated by the type field in the
header. Additionally, OpenFlow uses stream oriented transport and therefore must
indicate message boundaries in some way. The header's length provides this
mechanism and indicates the total number of bytes of the header and payload.
Figure~\ref{figure:ofp_msg_rep} shows a summary layout of the message.

\begin{figure}[h]
\begin{center}
  \includegraphics[width=.4\textwidth]{figs/ofp_pld.pdf}
  \caption{Value Directed Payload}
  \label{figure:ofp_msg_rep}
\end{center}
\end{figure}

The most interesting message is a Flow Modification. This allows for
the external modification of the data-plane of a switch device~\cite{ofp}. When a packet
enters the switch a flow table is consulted for a policy to apply to the packet.
The Flow Modification message allows for direct modification of this table. This
message begins with the standard header, with its type containing the
Flow Modification value 14. It is then followed by a payload that contains a 
match field, which specifies the conditions necessary for a packet match, and is
followed by various state information and a sequence of policy decisions, or
actions. Figure~\ref{figure:flow_mod_rep} summaries this payload structure.

\begin{figure}[h]
\begin{center}
  \includegraphics[width=.4\textwidth]{figs/ofp_flow_mod.pdf}
  \caption{Flow Modification}
  \label{figure:flow_mod_rep}
\end{center}
\end{figure}

\subsection{Representation Constraints}

This minimal example of message structure illustrates many common representation
constraints found in network protocols. Fields specify precise structural
constraints, either directly with bit precision, or indirectly through
dependencies. Simple integral types can have different representations (MSBF,
LSBF). It is useful to group like fields into aggregates such as the
header and match aggregates. Sometimes the type of a field is a choice based
on some previous value such as the message payload. Some fields are sequences
of types that can terminate implicitly (no more data available), or explicitly
based on some constraining length (header's length for example). Finally, these 
structures fall into one of two categories. They are either independent and we
know their precise structure without having to inspect a packet, or they are
dependent and their structure can only be surmised only after decoding some
prefix of the packet.


==> buffer_view_ops.tex <==
\begin{align*}
  view : ~&Ref(Buffer) \rightarrow View \\
  view : ~&Ref(View) \rightarrow View \\
  available : ~&CRef(View) \rightarrow Int \\
  advance : ~&CRef(View) \rightarrow Int \rightarrow View \\
  constrain : ~&CRef(View) \rightarrow Int \rightarrow View \\
  put : ~&Ref(View) \rightarrow CRef(T) \rightarrow Unit \\
  put : ~&Ref(View) \rightarrow CRef(Array(T,e)) \rightarrow Unit \\
  get : ~&Ref(View) \rightarrow Ref(T) \rightarrow Unit \\
  get : ~&Ref(View) \rightarrow Ref(Array(T,e)) \rightarrow Unit
\end{align*}


==> code_gen.tex <==
\section{Code Generation}
\label{code_gen}

After optimization and verification of invariants over the program, the compiler
will generate code. We currently support C++11 as our target language. All
message related type definitions and synthesized operations will be written to a
single set of .cpp and .hpp files, the program itself is written to main.cpp. We
use both language and library features of C++11 in order to simplify our output.


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

This paper presents the initial work of using programming language and compiler
techniques to improve the process of design, synthesis, and verification of
network protocols and systems. This work leverages the axiomatic systems
programming language Liz~\cite{liz}. Network protocols can generally be
abstracted into four orthogonal components: message, state machine,
configuration, and system interface. These four components present clear
boundaries and interfaces that allow for independent design, development, and
verification. While this paper is part of a larger project that aims at
supporting all of these components; this paper focuses on the difficulties 
of the message component.

The message layer of any protocol stack is notoriously difficult to get right.
The issues range from ensuring structural constraints (correctly indicated
lengths and kinds), performing representational transforms (correct byte
orderings), and ensuring semantic constraints (only uses defined values). A
survey of the US-CERT Vulnerability Database~\cite{us_cert} demonstrates
that mature organizations implementing mature protocols continue to make these
kinds of mistakes. Table~\ref{table:msg_tbl} demonstrates that this is not
merely an engineering problem. The cause is often the failure of a human to
carry out a systematic task, the careful implementation of the small set of
interfaces and constraints for a given message component. The failure of humans
to be systematic at a programming task is usually a clear sign for automation.

\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
  Proto. & Age & Bug Date & Vendor & Error & CERT \# \\ \hline
  \hline
  802.11i & 2004 & 2012 & Broadcom & value & 160027 \\ \hline
  OSPFv2 & 1998 & 2012 & Quagga & struct & 551715 \\ \hline
  NTPD & 1985 & 2009 & GNU & struct & 853097 \\ \hline
  ICMP & 1981 & 2007 & Cisco & struct|val & 341288 \\ \hline
  VTP & 1996 & 2006 & Cisco & value & 821420 \\ \hline
  Bootp & 1985 & 2006 & Apple & struct & 776628 \\ \hline
  \end{tabular} \\
  \caption{Message Related Vulnerabilities}
\label{table:msg_tbl}
\end{table}

This area has not gone unnoticed and has been developed in various
ways. When the wire-format is not important serialization solutions are
often used~\cite{asn, proto_buf}. However, with network protocols, because of
interoperability requirements, the wire-format is important. As a result a
series of DSL(s) that allow control over the wire-format
have been designed that synthesize data-structures and common operations using
correct by construction techniques~\cite{packet_types, datascript, binpac}.
Finally, language researchers have improved upon these DSL(s) with rich type
systems for ensuring some of the guarantees mentioned above~\cite{pads_orig,
next_700_ddl}. Additionally, some researchers have developed static analysis
techniques to survey existing code bases and find occurences of the above
mentioend mistakes~\cite{deputy}. Our work improves on previous approaches by
extending a systems programming language, and not just providing a DSL. This
allows for full program analysis providing stronger safety guarantees and
offering domain specific optimization that is exceedingly difficult to
accomplish by hand.

\subsection{Contributions}
\label{sec:contrib}

Message related vulnerabilities can be classified into one of three categories:
structural constraint violation, semantic constraint violation, and unsafe
access of conditionally present fields. Structural constraints relate to how a
message describes its shape or structure, the messages description may be
inconsistent with external knowledge. Semantic constraints relate to the
abstract value of a field, the value may be undefined. Unsafe access relates to
how the program interacts with a message and its fields, a conditionally present
field should not be blindly operated on.

Our system prevents these three categories of message related vulnerabilities. A
user writes a series of type declarations that model a message precisely. They
are then free to use a set of compiler synthesized operations in their program
necessary for message handling. The compiler will then ensure proper and
efficient usage of these operations throughout the user's program. C++11 is the
target language used in our compiler.


==> invariants.tex <==
\begin{align*}
  [ available(view) ~&\ge 0 ] \\
  [ read(variant) ~&\implies init(variant) ]
\end{align*}


==> prior_work.tex <==
\section{Prior Work}

The work reported in this paper differs from prior work in several
directions. First and foremost,
rather than address message handling with a Domain Specific
Language (DSL), we adopt a solution based on a general purpose language
expressive enough to capture structural semantics and value semantics
in an axiomatic style (see \secref{sec:foundation}.)
Second, safety is guaranteed by adopting declarative specifications 
instead of direct imperative programming.  Executable code is generated
from declarative specifications.  This yields
 correct-by-construction properties.  The generated (C++) codes can (and do)
use all sound, tried-and-true tricks from the imperative programming trade.
Instead of having to prove system programs written in imperative styles
--- a formible task in and of itself --- we prefer to capture key
properties and executable semantics in declarative forms, exposing
structures easily amenable to mathematical tools.  This approach
to network protocol proramming is novel, and is a key contribution of this 
paper.

PacketTypes~\cite{packet_types} is a first work towards developing a DSL to
handle the specific constraints of network protocol message formats. The
authors' motivate the work with the usual suspects of network protocol software
development: tedious, error-prone, ever-changing, etc. Users can specific binary
formatted network protocols in the PacketTypes overlay language. This language
is then compiled down to a C library. DataScript~\cite{datascript} is another
DSL that extended this idea to ad-hoc data format specifications. 
Binpac~\cite{binpac} can be viewed as an extension of
PacketTypes~\cite{packet_types}, where the authors' primary view is that
protocol message formats are merely a grammar problem, and seek
to generalize a format description language into a `data-model' with 
constraints. The generalization includes support for ASCII based protocols which
was not present with previous work~\cite{packet_types}. Specifications compile
to C++ libraries, and target applications are off-line packet capture analysis,
such as the Bro Network Security Monitor~\cite{bro}. PADS~\cite{pads_orig},
another DSL in this category, was the first work to use dependent type theory
~\cite{next_700_ddl} to show safety and correctness. Of all of these DSLs binpac
is the only project that is still known to be active. Rather than use a DSL
approach we extend a general purpose language to capture message structural and
value constraints. This allows for more comprehensive correctness and safety
guarantees.

Additionally, there is work related to using dependent type systems for
analyzing system programming safety, such as Deputy~\cite{deputy}. This work
focuses on reasoning over imperative programs for array bounds and tagged union
errors. Our approach differs significantly in that we axiomatize structural and
value constraints with a set of base primitives and then reason over declarative
specifications.


==> synth_ops.tex <==
\begin{align*}
  bytes : ~&CRef(T) \rightarrow Int \\
  to\_view : ~&Ref(View) \rightarrow CRef(T) \rightarrow Bool \\
  from\_view : ~&Ref(View) \rightarrow Ref(T) \rightarrow Bool \\
  equal : ~&CRef(T) \rightarrow CRef(T) \rightarrow Bool \\
  not\_equal : ~&CRef(T) \rightarrow CRef(T) \rightarrow Bool \\
  to\_string : ~&CRef(T) \rightarrow String
\end{align*}

